BOMs Away! Inside the Minds of Stakeholders: A Comprehensive Study of Bills of Materials for Software Systems

Software Bills of Materials (SBOMs) have emerged as tools to facilitate the management of software dependencies, vulnerabilities, licenses, and the supply chain. While significant effort has been devoted to increasing SBOM awareness and developing SBOM formats and tools, recent studies have shown that SBOMs are still an early technology not yet adequately adopted in practice. Expanding on previous research, this paper reports a comprehensive study that investigates the current challenges stakeholders encounter when creating and using SBOMs. The study surveyed 138 practitioners belonging to five stakeholder groups (practitioners familiar with SBOMs, members of critical open source projects, AI/ML, cyber-physical systems, and legal practitioners) using differentiated questionnaires, and interviewed 8 survey respondents to gather further insights about their experience. We identified 12 major challenges facing the creation and use of SBOMs, including those related to the SBOM content, deficiencies in SBOM tools, SBOM maintenance and verification, and domain-specific challenges. We propose and discuss 4 actionable solutions to the identified challenges and present the major avenues for future research and development.

==> Makefile <==
LATEXMK = latexmk

MAIN = main.tex
BIB=main.bbl
FIGURES = $(wildcard figures/*)
SECTIONS = $(wildcard sections/*.tex)
DEPS = $(FIGURES) $(SECTIONS) $(wildcard *.tex) $(wildcard *.bib)

main.pdf: $(DEPS)
	$(LATEXMK) -pdf $(MAIN)

clean:
	$(LATEXMK) -c $(MAIN)

distclean:
	$(LATEXMK) -C $(MAIN)


expanded.tex: $(DEPS)
	perl -pe 's/sigconf,review,anonymous/sigconf,anonymous/' $(MAIN)  > rip.tex
	latexpand --expand-bbl $(BIB) rip.tex > expanded.tex

diff.tex: expanded.tex
	perl -pe 's/looseness=[0-9\-]+//' expanded.tex  > expanded-clean.tex
	latexdiff first_submission/old.tex expanded-clean.tex  > diff.tex
#	perl -pe 's/looseness\\DIFadd{/DIFadd{\\looseness/' rip2.tex > rip3.tex
#	perl -pe 's/looseness=\\DIFdelbegin \\DIFdel{-2\n/-1/m' rip3.tex > diff.tex
#	perl -pe 's/looseness=\\DIFdelbegin \\DIFdel{-2\n}\\DIFdelend \\DIFaddbegin *\\DIFadd{-1\n}\\DIFaddend/-1/m' rip3.tex > diff.tex

#	patch diff.tex < fix.patch

diff.pdf: diff.tex
	$(LATEXMK) -pdf diff.tex


==> contents/results.tex <==

\section{Study Results}
\label{sec:results}

%\MAX{this one also goes in the results}  \os{Done}
% Addressed: I don't think we need this; let's save space
%It is unlikely that every security vulnerability will be addressed or that every best practice will be followed. Instead we must supplement attempts to secure upstream elements of the supply chain with management techniques lower in the chain. 

%We discuss the results of our study regarding SBOM creation and usage, challenges, and solutions. 


Nearly 60\% (84/138) of the study participants are familiar with SBOMs (see \Cref{tab:response_stats}). The 22 respondents from the "Critical" survey belong to 16 of the 102 (15.7\%) critical OSS.
%\trevor{We had responses from people from 16 of the 101 critical projects. Do we want to mention this?  We only had 22 participants.  That's a coverage of 15.84\%} \MAX{this goes in the results, just before addressing the research questions}

\input{contents/results/sbom_usage}
\input{contents/results/challenges}
\input{contents/results/solutions}

==> contents/results/challenges.tex <==

\subsection{\ref{rq:challenges}: SBOM Challenges}

We summarize and discuss the challenges of using and creating SBOMs, expressed by the participants.

% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{example-image-a}
% \caption{Challenges, people impacted, solutions, and solution providers \os{Added the placeholder for a nice figure or table showing challenges, people impacted, solutions, and solution providers}}
% \end{figure}



%\subsubsection{Common challenges} 
%\trevor{I don't think we need this subsection anymore; we merged all our challenges}
% Addressed: removed the subsubsection
%\nathan{Put all titles in bold w/ period at the end}
%done

%\dmg{not sure where to put this: did anybody mentioned the difference between source sbom and binary sboms?}\denys{agree, this would be a good one to mention if we have any. Also, this would be different to the ICSE paper?}\trevor{I went through all of our surveys and interviews and pulled all seemingly relevant quotes: see this document \url{https://docs.google.com/document/d/1U9ADP4W4omBIH4pN\_cLW2TINaEq9qbhzTt8qoooUfTw/edit}.  I figure we can add a challenge or add this somewhere else if we want} \nathan{this ties into dynamic SBOMs, which have pretty much been cut for time. Would be nice, but not sure we have room}\trevor{maybe in the extension?} \nathan{Added brief mentions of dynamic SBOMs and binary SBOMs to the "Keeping SBOMs up to date" and "Insufficient tooling" sections, respectively}



\begin{enumerate}[label=(\textbf{C\arabic*}), wide, labelindent=5pt]

  \item \textbf{Complexity of SBOM  specifications.}\input{contents/results/challenges/standard_specification}
  
  \item \textbf{Determining data fields to include in SBOMs.}
  \input{contents/results/challenges/fields_to_include}
  
  \item \textbf{Incompatibility between SBOM standards.}
  \input{contents/results/challenges/incompatibility}

  \item \textbf{Keeping SBOMs up to date.}
  \input{contents/results/challenges/sbom_drift}

  
  %\item \textbf{Versioning SBOMs with globally unique IDs.}
  %\input{contents/results/challenges/versioning}

  %\item \textbf{Generating global software IDs.}
  %\input{contents/results/challenges/software_ids}

  %\item \textbf{Little incentive to produce SBOMs.}
  %\os{Can we rephrase this one as little incentives to produce SBOMs?}\os{I did}
  % Moved to RQ1
  %\input{contents/results/challenges/upstream_motivation}

  % \os{merged into C1: complex specs}
  %\item \textbf{Confusing specs and lack of educational resources.}\input{contents/results/challenges/documentation}

  \item \textbf{Insufficient SBOM tooling.} 
  %\os{This challenge may be reduced quite a bit. It's not that novel anyway.}
  \input{contents/results/challenges/insufficient_tooling}

  \item \textbf{Inaccurate and incomplete SBOMs.}
  \input{contents/results/challenges/poor_quality_sbom}

  \item \textbf{Verifying SBOM accuracy and completeness.}
  \input{contents/results/challenges/verify_sbom}

  \item \textbf{Differences across ecosystems and communities.}
  \input{contents/results/challenges/differences}


  \item \textbf{SBOM completeness and data privacy trade-off.}
  \input{contents/results/challenges/privacy_protections}

  %\os{Not really a challenge, maybe we can include it in a discussion section}
  %\item \textbf{Component complexity.}
  %\trevor{We will put the cyber physical challenges here}
  %\input{contents/results/challenges/cps_complexity}


  %\item \textbf{Other challenges.}
  \input{contents/results/challenges/other}
      
  
\end{enumerate}

==> contents/results/challenges/cps_complexity.tex <==
While many of the challenges discussed pertain to software supply chain management, CPS must also contend with hardware supply chains. When asked about challenges facing CPSs, three of six respondents indicated that such systems are becoming increasingly complex, making it difficult to find components which can suit particular needs. One respondent noted that "[the] more [individualized cyber-physical systems] are, the more challenging the supply chain is in terms of identifying possible CPS that match the requirements and can be integrated in specified environment (e.g., w.r.t. interfaces, safety levels, parameterization)." 
%Furthermore, as one interviewee noted, procurement decisions in this field can come with a hefty pricetag, facilitating a need to ensure that components are adequate ahead of time: "sometimes even [within the] same domain... different scenario[s] can [lead one to] vary [their] choice of technology because those [components] are very expensive." 
With more complex components, it becomes more difficult for developers to determine their suitability for a given purpose, especially when project requirements can also be quite complex. Practitioners need a method of determining if and how components - both hardware and software - meet their specific needs and compliance requirements.\os{I found this challenge fuzzy, as I am not familiar with CPSs} \nathan{I see what you mean, but considering that we're marketing our exploration of other domains like CPS as an advancement from prior work, it might be prudent to try to include something dedicated to CPS/HBOMs}\dmg{I agree (fuzzy?relevant?), it does not seem to be about SBOM... } \MAX{that's the point.. the whole section talks about the difficulty in finding and selecting components}

Both the needs of consumers and the complexity of CPS components continue to increase. One respondent indicated that, even when adequate components exist, they may not be mature enough to be used in testing. Two respondents cited shortages of important components such as semiconductor chips that have impacted CPS development.

==> contents/results/challenges/differences.tex <==
\label{sec_differences}
Participants expressed a varying level of SBOM support across different package ecosystems and programming languages. One interviewee mentioned: "a big part of the bottleneck is just retrieving all the information that needs to go into the SBOM and getting it from different sources [...] some language communities do a better job of capturing the metadata [to] include in the SBOM."  Some respondents even suggested that tools from the same standard (\eg CycloneDX) drastically vary in quality across languages. As another participant mentioned, this "creates an ecosystem challenge for getting that data in an SBOM in a reliable way, because there are some data sources that you can't really trust." 

We also observed challenges of creating SBOMs for languages with limited or no package managers. A survey respondent mentioned: "For C/C++ projects, dependencies are typically defined in autotools or cmake files, and Node, Ruby, Python, Golang, etc all have their own dependency management systems; typically recording exact versions is an output of the build process, although this doesn't come "out of the box" with C/C++ projects".

25\% of critical project developers surveyed who were familiar with SBOMs listed a lack of language support as a deficiency in current SBOM specifications, while 8.7\% of SBOM practitioners agreed.  When asked about tool deficiencies, 41.67\% of critical project developers surveyed who were familiar with SBOMs expressed a need for more language specific tooling.

%Even tools from the same standard (\eg CycloneDX) drastically vary in quality across languages. "That's something that kind of seems to vary from language community to language community, \nathan{cut quote after here?} even within tools that are kind of currently maintained by the [redacted] teams themselves." 

%As one practitioner described the situation in an interview, "I think that a big part of the bottleneck is just retrieving all the information that needs to go into the SBOM and getting it from different sources... There are some language communities that do a better job of capturing the metadata [to] include in the SBOM."  

%They went on to describe a specific situation in which metadata essential to their use case was unavailable from the language API and so had to be obtained through ad-hoc channels \nathan{cut?}.  

%This "creates an ecosystem challenge for getting that data in an SBOM in a reliable way, because there are some data sources that you can't really trust." \nathan{restructure to highlight just the part about trust?}
%\MAX{in general it is long and hard to understand. Did anybody mention the difference between languages with and without package manager? I guess this is one of the key points} 
%\trevor{We have this quote from the survey: "For C/C++ projects, dependencies are typically defined in autotools or cmake files, and Node, Ruby, Python, Golang, etc all have their own dependency management systems; typically recording exact versions is an output of the build process, although this doesn't come "out of the box" with C/C++ projects"} \os{Added quote}



%Therefore, although language-specific tools may be the most suited for SBOM generation \nathan{cut? (are we arguing this explicitly?)}, it is important to ensure to developers the availability of tools to generate accurate SBOM regardless of the chosen language and technology. 

%Such an approach would also not address for proprietary platforms or languages for which no open-source tools exist. 

%Added a few words
%\trevor{this didn't come up in the survey, but we could potentially mention proprietary languages here. In theory they need SBOMs too, but open source tools likely won't support them.}



==> contents/results/challenges/documentation.tex <==
\dmg{why not merge with C1. it is about the same issue: the standard} \MAX{I agree!}
Our results show that, while documentation and educational resources exist for SBOM, their very technical nature make their adoption difficult. 
%One interviewee mentioned "It's not just simplicity in the spec. It's not simplicity in the tooling, but how we message it and how we communicate it. Because if we send them to the [standard] spec website, they'll take a look at that and go, well, I'm not going through all that work."  
When asked about deficiencies in SBOM specifications, 4 participants said they were confusing and 6 reported that the guidance was ambiguous.  Specification comprehension issues were brought up by 8.82\% of SBOM producers.
%when asked about the challenges they face.

The number of potential use cases and their associated fields make the specifications particularly daunting (see \ref{sec:over_spec}) as also mentioned by one interviewee:  
%The documentation becomes difficult to quickly parse, making it challenging for readers to learn those parts they really care about.  One expert had this to say, "One of the challenges will be how do we do the documentation in a way that 
"[...] if all you care about is security, you know, you can look that up very, very quickly and not be bothered by having to learn all these extraneous things that don't have anything to do with your use case."
\trevor{Originally we didn't think there was an interesting research opportunity here, but I think we could explore applying LLM's to documentation.  I mention this and provide a related work in the solutions section}\os{ok, then this one could be just one paragraph}

==> contents/results/challenges/fields_to_include.tex <==
\label{sec:fields}

While some fields (software versions, licenses, or component names) are commonly agreed upon, others depend on the use case. For example, practitioners seeking to analyze their software for vulnerabilities may require BOMs to link to an external vulnerability database. 

% \trevor{Put an emphasis on machine learning and cyber physical fields}

% \nathan{I'm just going to mention the top 5 choices here, since we gave them a list to choose from.}
% Addressed: I added a brief blurb to the bottom saying there's more

%including any preproccesing steps taken (13), descriptions of the training data (17) as well as descriptions for testing/validation data used (14), optimizers/loss functions used (13), the model structure (12), parameters (10), training environment (11), fairness issues (6), known/potential biases (8), other known problems (7), the presence of personally identifiable information (8).

Interesting is the case of BOMs for AI/ML.   Other than standard SBOM fields, 
%such as dependencies (15) and version number (13), 
the 20 respondents from this group pointed out fields such as descriptions of the training data (17) and validation/testing data (14), preprocessing steps taken on the data (13), dataset version (13), and used optimizers/loss functions (13). When asked about fields needed in DataBOMs, they highlighted data sources (18), data transformations (18), preprocessing steps (17), dataset size (16), known/potential biases (14), and data collection procedures (14).

\rev{Of the 6 CPS experts we surveyed, 3 expressed a need for part numbers, 2 testing and quality assurance data, 1 deployment information, 1 place of manufacture, and 1 limitations.}

\rev{Adding additional fields to SBOM specifications makes the documents more useful, but as mentioned previously, also contributes to the complexity of the specification (C1).}

%We see similar lists of unique fields for other BOMs (\eg HBOMs). \os{cut?}
%% [EXTENSION]
%% Expand on this
%% [EXTENSION]

==> contents/results/challenges/incompatibility.tex <==
% \dmg{I agree, it is long. I thihnk this section can basically say:
% \begin{enumerate}
%     \item each standard requires different formats, each format is difficult to compare/verify against the same info in another format/standard. even two tools that create the same standard format might generate radically different documents that are difficult to compare
%     \item competition creates confusion and uncertainty, but it is good at the same time;
%     \item there is ongoing effort to reach an agreement among different communities to unify SBOM formats.
% \end{enumerate}
% } \MAX{I added the last bullet, and then is fine. I also shortened the text below, if you want to keep the original} \os{sounds good}
Responses show that competing standards confuse developers. When consuming SBOMs, 23.33\% of the SBOM practitioners stated that different standards pose a challenge, due to  interoperability issues between standards and inconsistency between standards and tooling.
\looseness=-1
%Inconsistency in standards and tooling was mentioned by 30\%.  In the same survey, interoperability issues even impacted one producer \os{meaning?}.

%\trevor{I redacted the standard names for anonymity.  Is this needed?}
%\nathan{I removed this section: " I've learned some things from Standard A. I know Standard A has included stuff from Standard B... But " to save on space and avoid any missing context about where the interviewee works. In this context, the redaction isn't really necessary any more.}
%Addressed: Good call

Despite this, one expert said: "Competition is good [...] I definitely think that we have moved faster because of CycloneDX and SPDX having this kind of competition."  
%And another said, "I think the community will benefit a lot from having multiple standards. There's no one true approach, so there needs to be trial and error. It's a Darwinian process. [...] I don't think there will be a winner, [but] eventually, there will be interoperability."

%"I think the community will benefit a lot from having multiple standards. Because there's no one true approach, so there needs to be trial and errors. And it's a Darwinian process. There's no one true approach. And we need to have this kind of experimentation... I don't think there will be a winner. Eventually, there will be interoperability."

%\trevor{The next paragraph feels almost like a solution}
%Ultimately, the most important factor isn’t which standard is being used because "as long as [the BOM] is machine readable, it really shouldn't matter which standard becomes popular." \os{cut?}

%"So as long as it's machine readable, it really shouldn't matter which standard becomes popular or which one doesn't as long as they have a common interpreter to be able to represent what that dependency looks like."

%\MAX{I dropped the latter, doesn't say much, just format, which is a minor problem...}
%The problem is compounded when considering that the different standards also support multiple data formats.  One expert weighed in, "If you give me a piece of paper, if it's cardboard or Velen Premier paper. [...] That's paper, right? Doesn't matter what quality of paper you use. So first, we let go of supporting all these different formats. [Some standards] support both XML and JSON. And the XML and JSON format are subtly different... Less format would be more."\os{shorten substantially or cut?}

% Shortened for space
%"So first thing would be to let go of supporting multiple data formats. It's the same way, you know, I don't care if you give me a piece of paper, if it's cardboard or Velen Premier paper, or just [a] plain thing that we use on a typewriter. That's paper, right? Doesn't matter what quality of paper you use. So first, we let go of supporting all these different formats. [Some standards] support both XML and JSON. And the XML and JSON format are subtly different... Less format would be more."

There are also multiple ways of creating an SBOM for the same piece of software, often for backward compatibility reasons.  
One practitioner remarked: "You may have two SBOMs that technically represent the same software, but they're being produced by two different tools and they look radically different."  
%\os{this comment seems about tooling, not incompatibility of standards}\trevor{It's about the standard because the standard is what lets the tools create the SBOM in different ways.  Both ways can be "correct" so it isn't a tooling issue}
%Later they added, "Supporting too many use cases, too many possibilities, is not a good thing. So, simplification, slashing through, having fewer possibilities and having only one way to express something would be something that would help a lot." 
%And then, "It doesn't help with downstream usage and rationalization, especially [when] you expect an SBOM to be a format that favors and fosters normalization in a common format that's easy to understand and share between tools. It's not there. It's a problem. It's a serious problem." \os{shorten substantially?}

%\trevor{This also reads as a solution to the problem}\os{I think it is ok, it is an observation}
Fortunately, respondents suggested there are plans to increase and maintain interoperability among different standards.  As one interviewee put it, "I think [the standards are] on two different paths now. [...] To say one's going to die over the other, or try to do the grand convergence and bring them together, you're just not going to, it's just going to take too long. [...] it makes much more sense to try to get the two groups to collaborate."

%As one interviewee put it, "I think they're on two different paths now. [...] To say one's going to die over the other, or try to do the grand convergence and bring them together, you're just not going to, it's just going to take too long. I think it makes much more sense just to try to get the two groups to collaborate."

==> contents/results/challenges/insufficient_tooling.tex <==
\label{sec:insuff_tooling}
Figure \ref{fig:tool_support} shows
stakeholders' views on whether current SBOM tools address the needs of their users. While we generally found a lack of consensus among participants, we observe that tool makers are slightly more negative. These results, combined with the participants' open-ended answers, suggest that current tool support is insufficient. One participant identified a lack of "automated ways to generate SBOM for embedded code like assembly, C, C++." 
%\os{Add a small quote?}\denys{a quote ideally pointing out why one of the existing tools falls short?}
%Addressed: quote added

%Interestingly, tool makers have the harshest view of current tooling, but also  standard makers and educators lean towards a strongly disagree with the statement. Overall, there is a general feeling about the deficiencies of the available tool support

%The thoughts of consumers and producers are roughly the same.  Even though all groups agreed that current tooling is insufficient, Table \nathan{broken reference}\ref{tab:tool_awareness} shows that most tool makers disagree that stakeholders are even aware of the available tooling.

%Critical project developers were also asked their opinion on current tooling, but their responses interpreted in the context of the quasi-SBOM files that most participants referred to in their answers.


\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{images/tool_stats_smaller.png}
%\caption{Agreement for "Current SBOM tools meet user needs"}
\caption{Perceived sufficiency of SBOM tooling.}
\label{fig:tool_support}
\vspace{-0.37cm}
\end{figure}
%\nathan{Some survey name abbrevs are in square brackets, some in parentheses. Avoid referring to initial survey as "SBOM Survey," since they all examine SBOMs. Does "SBOM Practitioners" fit well? "SBOM Prac."?}}
% Addressed

% \begin{table*}[]
% \caption{Current SBOM tooling meets the needs of users} 
% \label{tab:tool_support}
% \begin{tabular}{|ccccccc|}
% \hline
% \multicolumn{1}{|c|}{Survey}                    & \multicolumn{1}{c|}{Role}              & \multicolumn{1}{c|}{Strongly Disagree} & \multicolumn{1}{c|}{Disagree} & \multicolumn{1}{c|}{Neutral} & \multicolumn{1}{c|}{Agree}   & Strongly Agree \\ \hline
% \multicolumn{7}{|c|}{Statement: Developers and stakeholders are aware of available SBOM tools}                                                                                                                                                   \\ \hline
% \multicolumn{1}{|c|}{SBOM Practitioner}                      & \multicolumn{1}{c|}{Tool Makers}       & \multicolumn{1}{c|}{12.50\%}           & \multicolumn{1}{c|}{37.50\%}  & \multicolumn{1}{c|}{16.67\%} & \multicolumn{1}{c|}{29.17\%} & 4.17\%         \\ \hline
% \multicolumn{7}{|c|}{Statement: Current SBOM tooling meets the needs of users}                                                                                                                                                                   \\ \hline
% \multicolumn{1}{|c|}{\multirow{6}{*}{SBOM Practitioner}}     & \multicolumn{1}{c|}{Across Roles}      & \multicolumn{1}{c|}{6.82\%}            & \multicolumn{1}{c|}{25\%}     & \multicolumn{1}{c|}{34.09\%} & \multicolumn{1}{c|}{22.73\%} & 11.36\%        \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{Producers}         & \multicolumn{1}{c|}{4\%}               & \multicolumn{1}{c|}{28\%}     & \multicolumn{1}{c|}{32\%}    & \multicolumn{1}{c|}{24\%}    & 12\%           \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{Consumers}         & \multicolumn{1}{c|}{3.23\%}            & \multicolumn{1}{c|}{29.03\%}  & \multicolumn{1}{c|}{29.03\%} & \multicolumn{1}{c|}{25.81\%} & 12.9\%         \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{Educators}         & \multicolumn{1}{c|}{7.14\%}            & \multicolumn{1}{c|}{21.43\%}  & \multicolumn{1}{c|}{28.57\%} & \multicolumn{1}{c|}{21.43\%} & 21.43\%        \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{Tool Makers}       & \multicolumn{1}{c|}{8.33\%}            & \multicolumn{1}{c|}{33.33\%}  & \multicolumn{1}{c|}{33.33\%} & \multicolumn{1}{c|}{20.83\%} & 4.17\%         \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{Standard Makers}   & \multicolumn{1}{c|}{7.69\%}            & \multicolumn{1}{c|}{23.08\%}  & \multicolumn{1}{c|}{30.77\%} & \multicolumn{1}{c|}{30.77\%} & 7.69\%         \\ \hline
% \multicolumn{1}{|c|}{\multirow{4}{*}{Critical}} & \multicolumn{1}{c|}{Across Roles}      & \multicolumn{1}{c|}{0\%}               & \multicolumn{1}{c|}{41.67\%}  & \multicolumn{1}{c|}{41.67\%} & \multicolumn{1}{c|}{16.67\%} & 0\%            \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{Producers}         & \multicolumn{1}{c|}{0\%}               & \multicolumn{1}{c|}{0\%}      & \multicolumn{1}{c|}{33.33\%} & \multicolumn{1}{c|}{66.67\%} & 0\%            \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{Consumers}         & \multicolumn{1}{c|}{0\%}               & \multicolumn{1}{c|}{50\%}     & \multicolumn{1}{c|}{25\%}    & \multicolumn{1}{c|}{25\%}    & 0\%            \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{Familiar Non User} & \multicolumn{1}{c|}{0\%}               & \multicolumn{1}{c|}{42.86\%}  & \multicolumn{1}{c|}{57.14\%} & \multicolumn{1}{c|}{0\%}     & 0\%            \\ \cline{2-7} 
% \hline
% \end{tabular}
% \end{table*}

% \begin{table}[t]
% \caption{Current SBOM tooling meets the needs of users} \os{How many responses?}
% \label{tab:tool_support}
% % \usepackage{multirow}
% \setlength{\tabcolsep}{2pt}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Survey                & Role              & SD & D & N & A   & SA \\ \hline
% \multirow{6}{*}{SBOM} & Across Roles      & 6.82\%            & 25\%     & 34.09\% & 22.73\% & 11.36\%        \\ \cline{2-7} 
%                       & Producers         & 4\%               & 28\%     & 32\%    & 24\%    & 12\%           \\ \cline{2-7} 
%                       & Consumers         & 3.23\%            & 29.03\%  & 29.03\% & 25.81\% & 12.9\%         \\ \cline{2-7} 
%                       & Educators         & 7.14\%            & 21.43\%  & 28.57\% & 21.43\% & 21.43\%        \\ \cline{2-7} 
%                       & Tool Makers       & 8.33\%            & 33.33\%  & 33.33\% & 20.83\% & 4.17\%         \\ \cline{2-7} 
%                       & Standard Makers   & 7.69\%            & 23.08\%  & 30.77\% & 30.77\% & 7.69\%         \\ \hline
% \multirow{4}{*}{KP}   & Across Roles      & 0\%               & 41.67\%  & 41.67\% & 16.67\% & 0\%            \\ \cline{2-7} 
%                       & Producers         & 0\%               & 0\%      & 33.33\% & 66.67\% & 0\%            \\ \cline{2-7} 
%                       & Consumers         & 0\%               & 50\%     & 25\%    & 25\%    & 0\%            \\ \cline{2-7} 
%                       & Familiar Non User & 0\%               & 42.86\%  & 57.14\% & 0\%     & 0\%            \\ \hline
% \end{tabular}
% }
% \end{table}

% \begin{table}[t]
% \caption{Developers and stakeholders are aware of available SBOM tools}
% \label{tab:tool_awareness}
% \setlength{\tabcolsep}{2pt}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% Strongly Disagree & Disagree & Neutral & Agree   & Strongly Agree \\ \hline
% 12.50\%           & 37.50\%  & 16.67\% & 29.17\% & 4.17\%         \\ \hline
% \end{tabular}
% }
% \end{table}

%The state of tooling is such an issue that when asked about deficiencies in the current SBOM standards, tooling was still the number one answer with 8 mentions (34.78\% of respondents).
%\nathan{Cut: kind of tangential}

Across stakeholder groups, there was little familiarity with tools. 85\% of the ML respondents were unaware of any tool support for generating AIBOMs, and 90\% were unaware of tooling for DataBOMs.  Only one CPS practitioner was aware of existing tools.
%This suggests that either such tooling does not yet exist, is insufficient, or is obscure.  All three present potential challenges to SBOM usage.

%Continuing the discussion from \ref{sec_differences}, tooling is generally language specific, meaning that the tool support for certain languages may be sufficient, while lacking for others.  
%\nathan{Cut: forward reference, plus the back half is kind of self-explanatory}
%It may be the case that developers have to build or improve tooling themselves, as was the case for one of our respondents, "So I might need to get in and kind of contribute to that library [Ruby CycloneDX implementation] in order to get it to where I need it to be for my purposes."
%\nathan{Cut: if tooling doesn't exist, it's implied that people would need to implement things themselves}

%The SBOMs generated by current tools may be missing fields or contain incorrect information, per challenge \ref{sec_poor_sbom}.  One respondent described their experience working with SBOM tooling as, "I have software that gives me a good start, but I have to go in and manually, based on my human-oriented findings of what's really in the software, I'll go in and edit it in that."  
%\nathan{Cut: forward reference, gets described later}
%Another described their experience, "there's a CycloneDX library that I've been using for Maven, or it's a Maven plugin that generates a CycloneDX file format. The way it outputs the SBOM, it doesn't differentiate between Maven sub-modules and third-party dependencies."
%Commented this quote out: a specific experience about a specific tool, plus we're already using a quote to describe this

Some projects with specific features may be unable to use current tooling, as no support exists for them yet. For example, \rev{one practitioner noted that current tooling couldn't "run fast on projects with tens of thousands of files...  They're not designed to work with very, very large projects."}  Two producers faced challenges involving projects that used multiple programming languages, 
%\denys{we can also abbreviate PL earlier and use this acronym. Will help saving/optimizing several lines}
suggesting an unmet need for tools to support multi-language projects.  Similarly, tools should be available for SBOMs to be created when only certain types of information are available, such as building SBOMs from binaries: "[T]here's source SBOMs. There's binary only SBOMs. There's SBOMs that have dependency information. There's SBOMs that have really just information about the package [...]." 
%This is a significant problem as many large software products have components written in more than one language.
%\nathan{Cut}

%One respondent described the problem, "[There are a] few tools and they don't really work well.  But again, nobody seems to care because maybe nobody's using them.  Or maybe they need to be better before anybody uses them better."  %It's chicken and egg.  So yeah, it would be nice to have some better tools."
%Shortened this

%While respondents identified various tools to produce SBOMs, in our interviews, multiple respondents expressed a comparative lack of tool support for SBOM consumption.

==> contents/results/challenges/low_adoption.tex <==

\rev{US Presidential Executive Order 14028 on Improving the Nation’s Cybersecurity requires companies selling software to the US government to provide corresponding SBOMs. This has created an important incentive at the end of the software development chain to create and maintain SBOMs; however, the results shown demonstrate that there are still many stakeholders that are yet to adopt (and in some cases know about) SBOMs. It is desirable that developers of open source libraries create and maintain SBOMs; however, while those consuming these libraries will benefit from such SBOMs, it is less clear how the developers of the libraries will benefit.} %Furthermore, at the current state, 
\rev{Creating SBOMs is not trivial and requires effort.  Without proper incentive, most developers forgo this effort.}

==> contents/results/challenges/other.tex <==
%\os{Is it worth making these their own challenge categories?}


%\os{I incorporated this into the RQ1 results}
%\item \textbf{Lack of formal guidance on distributing and sharing SBOMs - }
%In our survey of OSSF critical project developers, 5 of 12 respondents mentioned SBOM distribution as a challenge moving forward.  
%This made it the largest challenge from that group.  Additionally, one respondent from the SBOM practitioner survey also mentioned distribution as a major challenge.  
%Section \ref{sec:dist} describes how those surveyed would prefer SBOMs be distributed. 


\item \textbf{SBOMs for legacy packages and repositories.} One interviewee expressed the challenge of generating SBOMs for legacy software, which may be deployed and used by certain user groups.
\label{c:legacy}
%\os{cut this challenge? can this be merged with  keeping SBOMs up to date?} \trevor{I don't think that we can merge it with keeping SBOM up-to-date because they are pretty different.  I hesitate to get rid of it because this does come up in the solutions}\os{Fair enough}
Even if SBOMs become well-adopted and automatically generated during software builds, the question of what to do about legacy software remains.  Software that is still regularly maintained could feasibly have an SBOM created, but it is more challenging for older systems where the original source code is missing or for systems written in languages that are now substantially less common (\eg COBOL). These languages are less likely to be supported by open source SBOM tooling.  This is particularly problematic for entities like the US government \cite{legacy_in_gov} or the banking industry \cite{limaj2020facing}. \rev{It is possible that a community driven effort could generate and store SBOMs for such situations, but such a system is only theoretical.}

An important question is, whether, for existing systems, only the newest releases require an SBOM, or older releases that are still used by dependents also require SBOMs.  The respondent said: "if ecosystems did start to publish SBOMs, [...] it would be great to see [centralized repository maintainers] go back in time, generate SBOMs for older packages"

\item \textbf{Inability to locate dependencies for SBOMs.} 
\label{c:inabillity_to_locate}
%\os{This one has a direct impact on SBOM accuracy?} \trevor{Yes and no.  This is a distinct problem.  An SBOM can accurately describe a dependency, but if the reference is dead then there is no point. (That's one case)}
There may be cases where during the production or consumption of an SBOM, a certain dependency cannot be located.  This could happen if a dependency was removed from a package manager (perhaps it was malicious or no longer maintained) or from the associated repository.  One expert mentioned: "They [dependencies] may have been yanked and removed from the upstream package registries, meaning that the mere fact of detecting that they exist could be a challenge" and "In some cases, [finding your dependency is] a lost cause in the sense that your source may be dead, the repository has disappeared and you're left to have to sift through random snapshots of archive.org calls made on the website. That's rare, but that happens."  Previous work shows that malicious packages exist \cite{awssecrets, npmpackageshacker, pypimaliciousimage, pypiw4sp, bagmar2021know, chen2016following, top_5_challenges, zahan2021weak, liang2021malicious, sejfia2022practical} and are commonly removed from package managers once detected \cite{tenpackagesremoved}.  Since CVEs are for vulnerabilities \cite{whatiscve}, entries for malware are not typically created, potentially leaving developers with a dead dependency reference and little way to discover the security threat the dependency poses.

\rev{A simple solution here might be a centralized archive containing provenance information for software repositories and distributions indexed by global identifiers.  This would allow developers to access critical information for projects that are no longer hosted without requiring that source code be stored.  The storing of source code would be both expensive and potentially problematic in the cases of malware or proprietary software.}

%\nathan{merge "Industry pushback," "Fear of SBOM becoming a compliance document," and "SBOM is still a young technology" into "Barriers and Difficulties for Producing SBOMs?"} \nathan{merged}
%\item \textbf{Industry pushback.}
\item \textbf{Unclear SBOM direction and low adoption.}
\label{sec:unclear_direction}
\input{contents/results/challenges/low_adoption}

The Information Technology Industry Council \cite{iti} wrote an open letter in response to recent pushes from the US federal government to mandate SBOMs~\cite{object_to_sbom}.  They assert that SBOMs are not yet suitable contract requirements: "The presence of multiple, at times inconsistent or even contradictory, efforts suggests a lacking maturity of SBOMs."  
They also raise concerns about cloud services, legacy software \ref{c:legacy}, and the protection of confidential or proprietary information \ref{sec:privacy}, all issues mentioned by respondents during our study. Though, many of these concerns have also been addressed by the NTIA \cite{myths_and_facts}.

%\item \textbf{Fear of SBOM becoming a compliance requirement.} \nathan{It is a compliance requirement. The connotation we're going for is that we're worried people will think it's a *useless* compliance requirement, but we'll need to be more explicit about that if we don't merge this}\trevor{I had the same thought but was afraid the title for the challenge would get too long: what about SBOM becoming "useless" compliance document?}
This suggests a fear that the work required to create and maintain SBOMs will outweigh their benefits. As one of our experts said, "I hope that the hype around SBOM will lead to something that's productive [...] and will not just be something which is a compliance requirement that's going to be met in a minimal way.”  This fear was shared by  practitioners across domains.  Across our surveys, three respondents expressed worry that SBOMs would not be useful and other three feared that they would be time-consuming. 

%This excerpt from an ML survey response succinctly describes the challenge, "A major risk is that the BOM becomes "yet another" bureaucratic nightmare involving more and more documents to fill out, without actually solving the underlying problem"
%\item \textbf{SBOM is still a young technology.}
Lastly, as we were reminded by numerous respondents, SBOMs are still a young technology that will take time to mature. Currently, there is still a need to motivate and implement support for consumer use cases.  In an interview, one respondent stated, “You know, if you are a large organization and, say, you take a magic wand, and tomorrow all your software vendors start to provide accurate SBOMs, what are you going to do with this?”  %And another said, “I still don't know what to do with them in the sense that I'd like to know which product is used by Project 123. I don't care about SBOMs. I want an answer to these kind of questions.”\os{cut?}



==> contents/results/challenges/poor_quality_sbom.tex <==
\label{sec:poor_sbom}
%\dmg{perhaps merge with keeping them up to date? seems very related} \trevor{I agree that they are related, but I don't think they are the same challenge.  Maybe we could merge with tooling?  Since the poor SBOM is the result of insufficient tooling?}\denys{I would say this could also be a separate challenge as is, since in most of the cases inaccurate/incomplete SBOMs are the result of erroneous manual input?}
 An SBOM is only as good as the information that it provides. If the information is inaccurate or incomplete, it becomes difficult for teams to make informed decisions concerning the dependencies, licensing, and security of their projects. 
 %Often, generating high-quality SBOMs requires high-quality tools, which may not be available.
 
 According to the results, currently available SBOMs are of varying quality and are often found wanting. 33\% of SBOM consumers from the practitioner survey mentioned poor quality SBOMs as one of the challenges they had faced in using SBOMs. 25\% of the consumers from the OSS critical projects groups stated the same. Surprisingly, also 12\% of the SBOM producers had the same complaint.


Consider that the minimum SBOM requirement would be to include all direct and indirect \rev{(transitive)} dependency information, including the URLs of their sources. The legal expert we interviewed mentioned that, \rev{in his/her experience}, this condition is rarely met.
%the minimum SBOM standard to be including dependency information for direct and transitive dependencies as well as URLs to their source.  We asked a legal expert, who was also well versed in software, how many SBOMs met this condition in their estimation. The response was, "not very many."

%During an interview, one practitioner explained the importance of accurate information, “So in terms of hierarchy, I'd say security issues and the quality of vulnerability data is the most problematic. Second, licensing issues because each time you don't have accurate license information, you don't even know whether you can use it. And third, of course, provenance. I mean, you'll be able to find the correct corresponding source code if you have package metadata but the package doesn't tell you where to find the source. You need to search for that.” \os{Reduce substantially?} \MAX{rather drop, it does not add much} \os{Done}

\rev{Participants also discussed "false positives" in BOMs.  For example, just because your project uses a dependency and that dependency has a vulnerability, it does not follow that your project will necessarily be impacted.  It depends on the usage context of that dependency.  Determining if a project is actually impacted is a more difficult problem and will require more sophisticated tooling.}

The problem of inaccurate SBOMs also impacts tool developers. One respondent described how "it's been difficult to build tooling that accepts an SBOM when I'm not sure if all the fields that I'll need to depend on have been filled out."



==> contents/results/challenges/privacy_protections.tex <==
\label{sec:privacy}

%\dmg{these seem to be very domain specific... maybe gather all the AI/ML issues into one?} \MAX{it appears unclear how this is linked to the responses..} \trevor{We initially had this with separate ML challenges, but this is the only distinct ML challenge} \os{Grouping this one and The CPS challenge}
AI/ML participants indicated that AIBOMs and DataBOMs may entail a tradeoff between completeness and privacy on large datasets, given that these datasets may contain personally identifiable, private, sensitive, or proprietary information.  %This challenge also depends on how the data was collected and then processed. 
CPS respondents also mentioned privacy concerns in BOMs, as CPS may actively collect and process private and sensitive data from the environment.  \rev{Corporate entities have also expressed concern over exposing proprietary information through SBOM \cite{iti}.} 

%One of the areas where SBOMs require a tradeoff between completeness and privacy is the one of AI/ML-intensive systems, that inherently rely  on large corpora of data.  Sometimes these datasets contain personally identifiable, private, sensitive, or propriety information.  It depends on how the data was collected and then processed.  

%This is especially true for CPSs, \MAX{this looks a very strong statement, I would not claim that privacy issues in AI especially occur in CPSs} where data is actively collected from the environment.  
%Privacy constraints may
%make it difficult to create comprehensive and complete Data and AI BOMs.  As one respondent put it, "...privacy concerns could trump reproducibility concerns at times."

==> contents/results/challenges/sbom_drift.tex <==
\label{sec:update_sbom}

%\os{We may need more evidence here}\denys{agree, this is an important challenge}\trevor{I added some data from the survey in the last paragraph}
%Addressed: added a paragraph with data
Once an SBOM has been created, it must be maintained along with the software it represents. Substantial changes to an SBOM over time are known as SBOM drift~\cite{sbom_drift_1}.  These changes can happen suddenly. 
%even across different steps of the build process, the dependencies used by the software may change. 
For example, if a developer adds an application to a container, the number of dependencies can dramatically increase~\cite{sbom_drift_2}. Also, changes may even occur asynchronously from those to the software. For example, new vulnerabilities may be discovered in existing dependencies, which could affect SBOMs (if they contain vulnerability information)--- one interviewee described SBOMs as "a static vulnerability snapshot of the state of a [piece of] software at a certain point of time." 

\rev{When asked about deficiencies in standards, 4.35\% of participants expressed issues concerning keeping SBOM updated (1), upkeep requirements (1), and the syncing of SBOM versions (1).}  Of 3 critical project developers that consume SBOM, 1 mentioned difficulties in keeping SBOMs up-to-date. This motivates a need for tools which can dynamically update SBOMs as changes occur \cite{dynamic_sbom}.
%This highlights how SBOM drift can particularly affect systems which use SBOMs for security: as the landscape of known vulnerabilities and mitigations changes, the contents of a component's SBOM may need to change with them even if the component's software itself has not changed. 

%% Included info from the artciles & interviews
%% \trevor{this is likely related, but maybe not...}
%% SBOM drift \cite{sbom_drift_1,sbom_drift_2}
%% Sbom can be different at different phases of the build cycle

==> contents/results/challenges/software_ids.tex <==
% \dmg{I also think this is a major problem today, even if they are proposals
% but the important thing is that people mentioned it, so even if it is "solved"
% it is not deployed to the people who need it. but this section feels too long to say that.
% }
% \trevor{This one is interesting but a number of solutions already exist.  It may not be worth mentioning in the paper, maybe we save it for later.} \os{cut or reduce it to 1 paragraph?} \os{keeping it for now}
To make SBOMs actionable,  their dependencies must have their own globally unique identifier, and name collisions must be properly handled. 
%If there are collisions in the identification scheme, such as just using names, then it may become difficult, or impossible to determine which source your project is dependent upon.  
One interviewee mentioned: "If you're on the receiving end and trying to make sense, or trying to aggregate and combine the data from this different source, you're going to need some kind of identifier."

This is further motivated in that 30\% of SBOM practitioners listed software identifiers as a required SBOM field.  For comparison, that is only slightly less than the 32\% that listed dependencies as a must.  For both AI and Data BOMs, 50\% of ML practitioners, mostly unfamiliar with SBOM, selected unique identifiers as must-have fields. 

Due to the dynamic nature of security vulnerabilities, respondents also mentioned that SBOM should link to external vulnerability databases (\eg the CVE) rather than describing vulnerabilities.


Respondents also mentioned the importance to be able (using an accessible algorithm), to transparently generate a software ID once one has access to the software, and not using arbitrary IDs. While solutions in different standards exist, they are not interoperable yet.
%If the ID was arbitrarily assigned this would be difficult.  A scheme is likely needed that would allow you to determine the software ID by inspecting the software. \MAX{cut?}

%Solutions to this problem already exist, but in order for SBOM to become feasible, the usage of them most become more ubiquitous, and the interaction between different identification standards needs to be resolved.

%But when asked about generating globally unique IDs, one expert stated, "Oh, I think that's our hardest problem to solve, too, because what you want to do, you know, you're bringing information in from a number of different sources."

%"Otherwise, you have a really fuzzy matching algorithm that's imprecise, error-prone, and it has to be down to the specific version, not just the name of the package or the originator of the package.  So that, I don't think has been solved yet in the industry."\os{cut?}


==> contents/results/challenges/standard_specification.tex <==
\label{sec:over_spec}
%While participants expressed multiple deficiencies in SBOM specifications (missing data fields, under-specification, over-specification, missing use case support, and unavailable information), 
A common key concern among participants is the complexity of SBOM specifications, as stated in this comment: "[...] one core issue [...] is definitely a tension between use case coverage and the complexity of the spec." 
\looseness=-1

%: missing data fields (3), under-specification (3), over- specification (2), missing use case support (2), and unavailable information (1). 
%They expressed the following challenges with such specifications: large specifications (6), unavailable information (7), and under specification (1).

%A common concern among participants was the complexity of the SBOM specifications, as stated in this comment: "[...] one of the core issues [...] is definitely a tension between use case coverage and the complexity of the spec."  
%"I think, one of the core issues we have within the SBOM community is definitely a tension between use case coverage and the complexity of the spec." 
%While there are many fields that should be included in the ideal BOM, excessive fields may lead to increased complexity, lower adoption, and lower quality BOMs.  
When support for a new use case  is added to the specification,  the latter becomes longer and more complicated.
%, potentially leading to lower adoption and lower quality SBOMs. As
A standard maker mentioned: 
"[They say,] `the spec's too complicated.  All I want to do is X. [...] You're missing something for X, so I want to add that in,' which makes it more complicated for the other 99 people [without that use case]." 
%A critical OSS infrastructure developer remarked: "Standards are too stringent, I shouldn't need to consult a lawyer to list my code inputs." \MAX{if needed drop one example}

% \os{Not sure about his one (not very important?). Commenting it out for now. We may bring it back if necessary}
% If stakeholders perceive BOMs as just another requirement to fulfill, one interviewee suggested that developers may cut corners by filling in incorrect defaults or incorrectly copy-pasting from older BOM documents: "What are they going to do with the version number? They're going to type 'one'. Oh... the system didn't let me enter it, so [I'm] going to type 'two'."

%One of our experts had this to say: "At some point you have to ask, what are people really going to do with this information? What are they going to do with the version number? They're going to type one. Oh [...] the system didn't let me enter it, so [I'm] going to type two. [...] I guarantee you that's how people are going to use it."

%When asked about specification deficiencies, we found instances of practitioners complaining about missing fields (3), under-specification (3), over-specification (2), missing use case support (2), and unavailable information (1).  When asked about challenges faced, we saw the SBOM is too large (6), unavailable information (7), and under specification (1).

%\nathan{I think we we might have too many quotes in these next paragraphs}
%\trevor{I shortened some of the quotes}

%The problem is when support is added for a new use case, the spec becomes longer and more complicated. "[They say,] 'the spec's too complicated.  All I want to do is X. [...] You're missing something for X, so I want to add that in,' which makes it more complicated for the other 99 people [without that use case]." 

% I shortened the quote to save space
%"I get involved in conversations, I'd say at least on a weekly basis, where somebody says, the spec's too complicated. All I want to do is X. And by the way, you're missing something for my X, so I want to add that in, which, by the way, makes it more complicated for the other 99 people that aren't doing your use case."


We noticed that the user's perception of the SBOM specification is in part determined by their use case.  “If all you're interested in is licensing, you don't want to see all the security garbage in there. [...] Who cares what a vulnerability ID or a CPE is. [...] I don't want to have to learn all this just to be able to use the spec.”  However, "even if you, as a producer of an SPDX document, don't have that use case in mind, your consumers may have that use case in mind."

% Shortened the quote for space
%“So, the problem is that if all you're interested in is licensing, you don't want to see all the security garbage in there. [...] You know, who cares what a vulnerability ID is or a CPE is or all these other – in fact, I don't want to have to learn all this just to be able to use the spec.”  But then the problem is, "Even if you, as a producer of an SPDX document, don't have that use case in mind, your consumers, your customers may have that use case in mind."

%"It is a continual battle to fight the complexity because there definitely are contributors that have a model in mind that's much richer [than] the use cases that we support."\os{cut?}


%------------------------------

Participants also mentioned the lack of adequate educational resources about the SBOM specifications to better communicate their content. One interviewee mentioned: "It's not just simplicity in the spec. It's not simplicity in the tooling, but how we message it and how we communicate it. Because if we send them to the [standard] spec website, they'll take a look at that and go, well, I'm not going through all that work".
%When asked about deficiencies in SBOM specifications, 4 participants said they were confusing and 6 reported that the guidance was ambiguous.  Specification comprehension issues were brought up by 8.82\% of SBOM producers.
%when asked about the challenges they face.

%The number of potential use cases and their associated fields make the specifications particularly daunting (see \ref{sec:over_spec}) as also mentioned by one interviewee:  
%The documentation becomes difficult to quickly parse, making it challenging for readers to learn those parts they really care about.  One expert had this to say, "One of the challenges will be how do we do the documentation in a way that 
%"[...] if all you care about is security, you know, you can look that up very, very quickly and not be bothered by having to learn all these extraneous things that don't have anything to do with your use case."

==> contents/results/challenges/upstream_motivation.tex <==
%dmg{I think this should go to the discussion/conclusions} \MAX{Yes I'm wondering whether this is a challenge or a finding}\os{agreed}\denys{+1}
% Addressed: moved to RQ1
Participants expressed that the pressure to have SBOMs is largely felt by industry and projects at the end of a supply chain.  At present, there is little incentive for open-source projects towards the beginning of a supply chain to produce SBOM. Some projects, e.g., the Linux kernel, may have no real dependencies of their own and so do not require dependency management methods.  As one interviewee noted, "I don't see a rush to add SBOMs to the originating open source. I see a rush to add SBOMs to the middle folks..."

This results in downstream components creating SBOMs on behalf of their dependencies. Other than being a cumbersome task done for somebody else; as one interviewee said, "[the risk is] miss[ing] something because you got to go back and dig back through all these different dependencies."

%this presents another problem, as expressed during one of our expert interviews, "If you've got a dependency on a dependency on a dependency, none of those have SBOMs. And here you are in the middle of the supply chain trying to create an SBOM. You're going to miss something because you got to go back and dig back through all these different dependencies. And basically you're doing the work for what those dependencies should have done."

%In the realm of machine learning, we are likely to see a similar pattern emerge with the creators of large datasets, who will also be missing the inherent motivation to produce DataBOM.  Across our surveys, 2 respondents asserted that one key challenge for consumers will actually be acquiring BOMs from other projects.  One respondent went so far to say, "In industrial settings, we mostly assume SBOMs are unavailable." \MAX{I cut this, nothing specific to AI/ML}

%When asked how we can make SBOMs easier to use, one interview respondent stated, "I think right now, just generating the SBOM, like if the SBOM was already available [from the provider], then I wouldn't have to generate it."\os{cut?} 

==> contents/results/challenges/verify_sbom.tex <==
\label{sec:verify_sbom}

33\% of the OSS critical infrastructure contributors mentioned how SBOM verifiability is a major challenge. This was also reported by 3 participants of the SBOM practitioner survey.


%During an interview, one participant said, "I think [the consumer] inherently has to trust the content of the SBOM as accurate [...] If the consumption tools can't really trust the content, then they're going to have to go get the data themselves from somewhere else, which is what the generation tools have to do. So then it kind of defeats the purpose of the file format in the first place." \MAX{this example can be dropped} \os{Dropping it for now}

That being said, the enforcement of SBOM correctness should not be so strict that it impedes SBOM creation and adoption. For example, the legal practitioner we contacted cautioned that holding BOM creators liable for inaccuracies in the documents they produce is a disincentive to creating SBOMs at all. 

\trevor{We can trim this, but this is a finding we should mention}
\rev{For security reasons, it will also be necessary to validate the integrity of BOMs.  Consumers will need mechanisms they can use to verify that the BOM they have received is actually the one produced by the software provider and that no other actors have mutated it in transit.  Integrity checking is a common cybersecurity problem with well-understood solutions, like hashing, that can likely be applied to this context as well.}

==> contents/results/challenges/versioning.tex <==

SBOMs should have unique version identifiers just like the software that they represent.  These SBOM versions are not inherently tied to changes in the underlying software however, but instead to changes made to the SBOM document itself.  Given that current tooling often misses or inaccurately fills certain fields, it is sometimes necessary to manually and retroactively correct an SBOM.  At this point, there are two SBOMs, nearly identical, that represent the same build.  It becomes crucial to have mechanisms to properly and appropriately maintain and manage these SBOM versions.  One interviewee described the problem: "In theory, you generate a new globally unique ID every time you produce an SBOM.  What I find in practice is most people don't do that. [...]  According to the spec, it's supposed to be absolutely unique.  You change one character in that SBOM, you should change the globally unique ID for that."  Without these globally unique identifiers it can become challenging for clients to determine which version of an SBOM they have on file.


% \dmg{I am not sure about this one: why do we need versions of SBOMs? different variants (not versions? if it is about a better version of an SBOM, then the problem is one of uniquely identyfing (in the whole universe) an SBOM to make it that, if two files have the same id, they refer to the same information of the same software at the same version, (even if created by two differenot people?}
% \trevor{this one isn't super interesting and it's solutions are pretty trivial (better tooling).  We may be able to save it for the extension} \os{cut!} \MAX{either cut or paraphrase the response below.. too long for that it says}
% \trevor{SBOMs need to be versioned so that if changes are made you will know which version you have.  There may be 10 versions of SBOM for the exact same software build (maybe information was found to be incorrect and was fixed).  You need to know if you have the correct, newest SBOM.  That's the problem here.  That and people don't actually do the IDs right.}
% Ideally, a new SBOM version with a globally unique ID needs to be issued whenever there is a change made to the document, regardless of if any change was made to the underlying software.  An interviewee said: "In theory, you generate a new globally unique ID every time you produce an SBOM.  What I find in practice is most people don't do that. They may increment the version number on it, but I think we do have a problem. [...] According to the spec, it's supposed to be absolutely unique.  You change one character in that SBOM, you should change the globally unique ID for that."


==> contents/results/sbom_usage.tex <==

\subsection{\ref{rq:usage}: SBOM Creation and Usage}

\subsubsection{SBOM awareness and formats} 
\input{contents/results/usage/formats_adoption}

\input{contents/results/challenges/upstream_motivation}


\subsubsection{SBOM use cases, benefits, and data fields}
\input{contents/results/usage/use_cases}


\subsubsection{SBOM generation process, tooling, and distribution}
\input{contents/results/usage/tooling}
%\input{contents/results/usage/distribution} \nathan{merged into tooling}

==> contents/results/solutions.tex <==

\subsection{\ref{rq:solutions}: Solutions to SBOM Challenges}


\begin{table}[]
\caption{Relationships btw. challenges,  solutions, and roles.}
\label{tab:challenges}
\setlength{\tabcolsep}{2pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c}
\hline
\textbf{Challenge}               & \textbf{Solved by }                      & \textbf{Depends on}                                                                           & \textbf{Affected}               & \textbf{Who can fix it} \\ \hline
\multicolumn{1}{c|}{C1}  & \multicolumn{1}{c|}{S1}         & \multicolumn{1}{c|}{C2, C3}                                                          & \multicolumn{1}{c|}{P, C, TM} & SM, E          \\
\multicolumn{1}{c|}{C2}  & \multicolumn{1}{c|}{S1}         & \multicolumn{1}{c|}{C9}                                                              & \multicolumn{1}{c|}{P, C, TM} & SM             \\
\multicolumn{1}{c|}{C3}  & \multicolumn{1}{c|}{S2}         & \multicolumn{1}{c|}{-}                                                               & \multicolumn{1}{c|}{P, C, TM} & SM             \\
\multicolumn{1}{c|}{C4}  & \multicolumn{1}{c|}{S2}         & \multicolumn{1}{c|}{C5}                                                              & \multicolumn{1}{c|}{P, C}     & P, TM          \\
\multicolumn{1}{c|}{C5}  & \multicolumn{1}{c|}{S2, S4}     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}C1,C2,C3,\\ C6,C7\end{tabular}}       & \multicolumn{1}{c|}{P, C}     & TM             \\
\multicolumn{1}{c|}{C6}  & \multicolumn{1}{c|}{S1, S2, S3} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}C4, C5, C9,\\  C10, C11\end{tabular}} & \multicolumn{1}{c|}{P, C, TM} & P, TM          \\
\multicolumn{1}{c|}{C7}  & \multicolumn{1}{c|}{S2, S3}     & \multicolumn{1}{c|}{C6}                                                              & \multicolumn{1}{c|}{C}        & TM             \\
\multicolumn{1}{c|}{C8}  & \multicolumn{1}{c|}{S1, S2}     & \multicolumn{1}{c|}{C5}                                                              & \multicolumn{1}{c|}{P}        & TM             \\
\multicolumn{1}{c|}{C9}  & \multicolumn{1}{c|}{S1}         & \multicolumn{1}{c|}{-}                                                               & \multicolumn{1}{c|}{P, C}     & SM, TM         \\
\multicolumn{1}{c|}{C10} & \multicolumn{1}{c|}{-}          & \multicolumn{1}{c|}{-}                                                               & \multicolumn{1}{c|}{P}        & -              \\
\multicolumn{1}{c|}{C11} & \multicolumn{1}{c|}{-}          & \multicolumn{1}{c|}{C8}                                                              & \multicolumn{1}{c|}{P}        & -              \\
\multicolumn{1}{c|}{C12} & \multicolumn{1}{c|}{S4}         & \multicolumn{1}{c|}{C1, C3}                                                          & \multicolumn{1}{c|}{P, C}     & SM, E  \\       \hline
\end{tabular}
}
{\footnotesize Role: P=Producer, C=Consumer, TM=Tool Maker, E=Educator, SM=Standard Maker}
\end{table}



In this section, we discuss solutions for the identified challenges.


\Cref{tab:challenges} shows the identified challenges and, where applicable, which proposed solutions would address them.  We also include information on the stakeholders impacted by the challenge, as well as those that could be part of a potential solution. \rev{The challenges enumerated previously do not exist in a vacuum.  Instead, they feed into each other creating an interconnected web of dependencies.   We observed these connections early in our investigation, but formalized them through rigorous discussion and analysis after distilling our list of main challenges.  Discussions focused on the root causes of challenges as well as what impacts solutions might have.  Knowing these dependency relationships can help research teams better decide where to focus their efforts.}  The table also reflects these dependencies.  The current solutions identified do not address \ref{c:legacy} and \ref{c:inabillity_to_locate}: these will require additional research to mitigate effectively. % The challenges don't exist in a vacuum, and some may influence others.  This dependence relationship is also seen in the table.

%\newcounter{s_count}
%\newcommand{\scounter}{(S\arabic{s_count})}

\begin{enumerate}[label=(\textbf{S\arabic*}), wide, labelindent=5pt]

    \item \textbf{Multi-dimensional SBOM specifications.}
    \input{contents/results/solutions/data_levels}
    
%\refstepcounter{s_count}
    \item \textbf{Enhanced SBOM tooling and build system support.}
    \input{contents/results/solutions/better_tooling}
    \input{contents/results/solutions/add_to_tooling}

    %\item \textbf{Better tooling.}
    

    %\item \textbf{Open sourcing SBOM creation.} \os{cut whole solution?} \MAX{I agree, it is mostly already there}
    %\input{contents/results/solutions/opensource_creation}

 %\item \textbf{Enhanced accuracy and completeness of BOMs.}
    \item \textbf{Strategies for SBOM verification.}
    \input{contents/results/solutions/verify_sbom_solution}

    %\item \textbf{Generating globally unique identifiers for software.}
    %\input{contents/results/solutions/software_id_solutions}

    \item \textbf{Increasing incentives for SBOM adoption.} %\os{can we also make this about "increasing incentives"? }\trevor{I think we could add that here} \nathan{updated title}
    \input{contents/results/solutions/catch_all}
    
\end{enumerate}




==> contents/results/solutions/add_to_tooling.tex <==
%\dmg{the title should be: Adding support for SBOMs to ... and i would rephrase it: build systems should be SBOM aware: able to read and generate SBOMs and the section can be shortened without removing any insights and the next (Better tooling should be merged with this... it is part of the same problem}
%% Add to build tools
In addition to enhanced tool support, existing build systems (\eg Maven or Gradle) should be made SBOM-aware: capable of reading and generating SBOMs.  As one practitioner put it, "one way [for SBOMs to be easier to use] would be for build tools to start generating them without asking."  We have observed from our surveys that developers tend to prefer processes or tools that are commonly used or predetermined: "when the recommended way of doing something is the default, then it gets done more often."  Including SBOM generation functionality in build tools would more easily facilitate the update of SBOMs \ref{sec:update_sbom} and their versioning \trevor{versioning challenge}.
%, and their distribution along with software packages.

%While a step in the right direction, the solution relies on Dependency Graph, which has good, but limited language and ecosystem support \cite{dependency_graph}.  
%\MAX{I have used these tools, but I don't get the challenges in integrating them in build systems. I've seen projects where they are already called in Maven pom or in GitHub workflows}

%% Add to package managers
We have seen that developers rely on package management systems to obtain a list of their project's dependencies.  Many of these systems also provide quasi-SBOM files.  If SBOM generation and acquisition could be handled at the package manager level, we would likely see a large uptick in adoption \ref{sec:unclear_direction}.  SBOMs could be stored along with other package information and queried through APIs.  
%Now if package managers don't also generate the BOMs, then it may be best if they provide pointers to them.  This is because 
Indeed, interviewed  practitioners suggested that SBOMs should be kept as close to the source as possible.  As an SBOM moves further from the source, it is less likely to be up-to-date \ref{sec:update_sbom}.

GitHub recently unveiled new functionality capable of generating SPDX documents for a cloud repository \cite{github_tool}. Through integration with GitHub's Dependency Graph tool \cite{dependency_graph}, this capability supports SBOM generation for a number of popular languages and is easily accessible to developers, marking a strong start for SBOM integration.
\looseness=-1

%This isn't unheard of as Maven Central requires POM files for packages to be published.

%One respondent had this to say, "And I do think package managers are a key to this."

%% Add to other tools like pytorch and tensorflow
It was also suggested that ML libraries could generate AIBOMs or play an integral part in easily accessing the information required during generation. "I imagine[...] that eventually there'll be [...] something built into TensorFlow or PyTorch
[...] that outputs a document in a JSON file [...] that tells you the
key elements [like] the hyper-parameters."

==> contents/results/solutions/better_tooling.tex <==
%\dmg{merge with previous. they are the same issue, or perhaps the difference is "better tooling to consume/use sbom" (see my comments about what to use sboms for} \MAX{I agree! }\denys{agree as well}
% Addressed: merged
Across all surveys, three respondents suggested better libraries as a tooling solution.  One said, "Increased investment in open source libraries that can be incorporated in end user commercial and open source tools [can address current deficiencies in tooling]."  These libraries would serve as the foundation to develop SBOM tools \ref{sec:insuff_tooling} providing functionality for creating, maintaining \ref{sec:update_sbom}, parsing, and managing SBOMs, enhancing the user experience and potentially SBOM adoption. 
%For example, tools can be developed to support multiple ecosystems. 
%At the same time, tool developers could also enhance  language-specific support.
%\MAX{this point looks very generic, it does not add much in term of knowledge. I'd drop it}

Our findings indicate the need for language-specific SBOM production tools. A language-agnostic tool is unlikely to adequately support all scenarios. As such, there is work to be done creating SBOM generation tools for different ecosystems, including resolving disparities in the quality of available tools. Creating better tools will be a community effort: "part of it is just [...] being willing to get in and help out with the quality of those tools."  Language-specific tooling can be built on language-agnostic libraries \ref{sec_differences}. 

% Pulled from verification
\rev{SBOMs will likely become more accurate and complete with better tool support \ref{sec:poor_sbom}. Respondents from the critical projects survey pointed out that quasi-SBOM files are typically accurate  and are generated/checked automatically by tools: mature SBOM tools would likely be able to perform similarly.}

%\MAX{shouldn't this go under the solutions related to verification of SBOMs?}
% Addressed: moved
% I moved this to tooling, but the solution is really better tools
\rev{Moreover, in the current landscape of varying SBOM quality, consumption tools may also be responsible for checking the accuracy of the SBOMs consumed \ref{sec:verify_sbom}.  A respondent noted that consumption tools "have a perhaps harder job to make sure that the data that's being generated is accurate."} %"And so I think, you know, those tools [consumption tools] have a perhaps harder job to make sure that, that they're, the data that, the data that's being generated is accurate."

Developing well-maintained and easy-to-use SBOM libraries that can be leveraged by the community can boost community engagement in delivering improved SBOM tools.
%Instead, it makes more sense for tools to be specialized to handle the challenges present within particular languages and environments.
%\dmg{I would say you need both: some language aware, some language agnostic, depending on whether their use is language agnostic or not: a verification tool needs to language aware, a tool to compare two sboms can be agnostic, etc.}
%\MAX{maybe we should just report what the respondents said}
%\trevor{The language agnostic (consumption) tooling is mentioned in the next paragraph}


%\nathan{Cut this paragraph: it's trivial that consumption tools consume SBOMs of a certain format and that formats are independent of programming languages, so as long as we're clear elsewhere that tools need to produce high-quality (i.e. interoperable) sboms, we're good}SBOM consumption tools, however, should be language agnostic, as it makes little sense to have tools that are only capable of consuming SBOMs from one language community. Also, software systems could be multi-language.  %Standards and consumption tools should be as language agnostic as possible.
%One respondent commented that "I could use that tool to generate an SBOM and then I could use the SBOM as kind of my common file format for computing the metrics that I'm interested in." \MAX{not sure the example adds much, it could be dropped}



%One respondent mentioned a system to help identify what data fields tools are capable of reading and producing. They likened this system to how different browsers, and versions of those browsers, support HTML tags, CSS, and JavaScript.  Perhaps an online resource, like those that exist in that space, could add clarity to the capabilities of existing tooling and help developers make informed decisions about which tools fit their use cases. \MAX{candidate to drop} \nathan{paraphrased below}

%\trevor{cutting for space}
%One respondent suggested that a central resource (\eg a website or repository) might help identify tool capabilities. Such a resource would effectively communicate which data fields SBOM tools are capable of reading or producing, helping developers to make informed decisions about which tools fit their use cases.



==> contents/results/solutions/catch_all.tex <==
There is a need to either minimize the effort needed to
create and maintain SBOMs (such as improving current development toolkits to generate them) or by gaining other benefits, such as having tools that consume SBOM and help with developer tasks. Similarly, it is
necessary to motivate the creators of the development toolkits to support SBOM creation \ref{sec:insuff_tooling}. Github's new SBOM tools are a
step in the right direction. Also, issuing badges might be a simple incentive that might promote the adoption of SBOMs (as it has been in other domains \cite{DBLP:conf/icse/TrockmanZKV18}) \ref{sec:unclear_direction}.

Similar to Executive Order 14028, other stakeholders could require their participants to provide SBOMs. For example, the scientific publication of tools and models could require that artifacts be accompanied by SBOMs \ref{sec:unclear_direction}. These SBOMs would increase the transparency of the work and ideally increase reproducibility.

At the same time, better marketing and educational materials that emphasize the importance of SBOMs are needed, not only for those that create the software but also for those that consume it.  As one user put it, "It’s not just simplicity in the spec [nor] simplicity in the tooling, but how we message it and how we communicate it."

Ultimately, creating and using SBOMs should be done because it helps to create and maintain better, more secure, and reliable software, and that ultimately benefits society.

%\dmg{the text below is the old one}


%From our study results, it is clear that all SBOM stakeholders (producers, consumers, and tool makers) need more incentives to increase SBOM adoption. The solutions we have discussed in this section can assist in achieving this goal.

%Better marketing and more effective communication about SBOMs is required.
%Effort needs to be invested in distinguishing  SBOMs from other dependency-tracking systems and quasi-SBOMs, or making clear how these can interoperate.  It is also possible that advances in large language models can be used to facilitate writing clear, more user-friendly specifications \cite{stripe_gpt}. This technology could also be used for retrieving facts about the specification with examples of SBOMs for different usage scenarios and contexts. 

%The importance of good marketing and design decisions cannot be overstressed.  As one user put it, "It's not just simplicity in the spec [nor] simplicity in the tooling, but how we message it and how we communicate it."

%In our surveys with ML and CPS practitioners, many expressed concern about the adoption of SBOMs, some putting forward requirements as an incentive for developers.
%For example, if academic conferences required completed SBOMs to accompany deep learning models or other novel solutions.  These SBOMs would provide transparency into the work and ideally increase reproducibility and potentially facilitate faster research outcomes.

%Other incentive strategies will likely need to be applied to encourage open-source developers to produce SBOMs for their projects.



% \dmg{One idea: do all these Sn points and at the end finish with the need to have
% incentives as the overall arch: incentives for those that create them, and incentives for those that use them. the idea of having a tool that can verify in an SBOM is accurate and verify if there a CVE on that software sounds like a really needed one.}


==> contents/results/solutions/data_levels.tex <==
%\dmg{why? BOM? continue to talk about SBOMs so there is consistency} \MAX{I agree, even if these are Data or AI BOM or HBOM, it's fine to talk about SBOM not to confuse with BOM in general}
%\dmg{II would call the section: Different types of SBOMS and different compliance levels. not sure about the use of the term "Data Levels" (at least for me it does not ring a bell)}\denys{agree with Daniel's comment}
We identify three dimensions that contribute to the complexity SBOM specification: (1) the intended use case of an SBOM, (2) the type of software the SBOM is generated for, and (3) the amount of information documented in an SBOM.  Providing clear guidance for these dimensions is needed to inform consumers/producers which fields an SBOM should contain \ref{sec:fields}. The ultimate goal being to reduce the cognitive load placed on users of the specification \ref{sec:over_spec}. %Next, we discuss these three dimensions.

%Determining the answers to these three questions will inform producers regarding the fields that the produced SBOM should contain.  The goal should be to reduce the cognitive load placed on the users of the specification.

%\trevor{why is this in bold?}
%\nathan{The doc of SPDX use cases we got lists 17... I know it's far from complete by their own admission, but do we want to go with "hundreds?" \url{(https://wiki.spdx.org/view/Technical_Team/Use_Cases/2.0)}} \os{addressed}
\underline{SBOM use cases.} There are dozens of potential use cases for SBOM~\cite{spdx_use_cases}, many already discussed. Including solutions for all use cases would clutter the specification (see \ref{sec:over_spec}).  In interviews, we learned that the SPDX team is working on \textit{profiles} \cite{spdx_why_security} which define the fields required in an SBOM document meant for a specific use case. This will allow producers to create SBOMs tailored for their use case without worrying about fields that to them are irrelevant.  One practitioner mentioned that "being able to call [use case] out in these profiles will make [what to expect in the quality] a lot clearer. And I think that might help with [poor quality SBOMs] \ref{sec:poor_sbom}. Not so much making the quality of the SBOMs better, but at least making it obvious what the quality is."  Another said: "Let's say I want to just graph the relationships, right? There's a lot of data that's included in the SBOM that I wouldn't necessarily need. And if some of that data is expensive to calculate, then the tool that gives me the SBOM would run a lot faster if all I was ever looking for was a way to kind of graph the relationships." 
%\os{Should we mention that cyclone sboms are kind of extensible (with user based fields or something like that)?}
%\dmg{ok, so (compliance) levels in this context really mean one level is a superset of the previous ones. I think this is orthogonal to the use of different types of SBOM} \os{commenting this out for now, but may be interesting to talk about "compliance"}
%\MAX{maybe if we need space, just take the first one, more related to the problem} 

%\dmg{software types? should it be types of software?} \nathan{agree, wording is confusing. why is it bold?}
\underline{Types of software.} Different types of software require different information to adequately describe them.  ML-related software requires fields that firmware or cloud services likely will not.  Even though all three fall under the umbrella of software, it may be prudent to separate them into distinct SBOM types (AIBOM, FBOM, SaaSBOM, \etc), so that it is easier for end users to know the type of system the SBOM describes. This model of different SBOM types has already been adopted by CycloneDX~\cite{cyclone_capabilities}.

%"You can't use SPDX with firmware as it's just too large."

%This would also make learning the spec easier, users would only need to learn the fields related to the type of BOM they need. 


\underline{Amount of information in SBOMs.} Within the same use case and software type, users may desire different amounts of data in an SBOM.  One practitioner noted:
%It could also be that some data is simply unavailable, is hard to obtain, or would reduce the incentives for developers to create SBOMs, meaning that true completeness is not always possible.  Here we introduce the idea of a data level, as brought up by one of our practitioners. "So it's pretty easy to generate a valid CycloneDX file that has almost nothing in it. 
"it would be interesting to have different levels [...] where this has `level 1' data. [...] This tool generates `level 2' data, this tool generates `level 3' data...".
These data levels reflect the amount of information a user can expect to find in the SBOM.  \rev{Lower data levels could potentially be used for privacy sensitive applications \ref{sec:privacy}.}
%That is, a level 1 BOM might only have the minimal field, where as a level 3 also contains information for all the optional fields for a particular use case.
%There may be cases where we "don't try to put everything in [the BOM]. Just put these like five or six key things that help the downstream know what the heck you built."
%\MAX{the next 3 paragraphs could be candidate for a radical shortening, or even removal} \nathan{done: see below}
Data levels could also create some standardization in tooling: %"So for a tool to say, hey, we only generate the bare minimum, or for a tool to say, hey, we only generate complete data set, then I think it would help people who are writing tools and adjusting those file formats to be able to then differentiate between the level of data that they can expect to see within the SBOM." \nathan{shortened}
"I think it would help people who are writing tools [...] to be able to then differentiate between the level of data that they can expect to see within the SBOM."

%The concept of data levels can also be applied to the generation steps of an SBOM.  "If you did look at different levels, it could be that the compiler spits out a `level one'. But then you can run a tool that adds `level two' data, and you can add another tool that adds `level three' data. And it could be that they get [successively] more expensive." \nathan{Cut: this doesn't add much to the data levels concept beyond combining different tools together}

%For example, you could describe an SBOM as: Level-1 licensing AIBOM. From this alone, you know that the SBOM is intended for licensing activities on an AI component, and fields unrelated to those purposes may not be required. \nathan{Cut: above is already clear}

Adding this flexibility to standards does not necessarily make them more complex or difficult to use. One practitioner indicated that "even though the minimum requirements that have been provided [...] seem to be or could be construed as daunting, the essence of what needs to be provided in SBOM can be surprisingly simple." Educational resources and documentation will have to be well-crafted to explain this approach.  

% Not sure that we actually need this
%Further research should  better understand the interplay between these three (and other) dimensions and to determine which fields should be included in which circumstances.
%, however this work presents the a significant step in that direction.

% \trevor{I'm not sure where this should go}
% \nathan{Since it's not meant to be a serious standard, maybe cut it? We have plenty of material already arguing for simplicity.} \os{yeah, cut!} \os{Done!}
% In our investigation, we came upon the Keep It Simple SBOM (KISSBOM) standard \cite{kissbom}.  While intended as a tongue in check standard, it still puts forward sound philosophy on the considerations that should go into standard creation.

==> contents/results/solutions/opensource_creation.tex <==

\dmg{I think you mean: Open sourcing SBOMs, you don't open source processes
but I think the key here is not to open source a project that creates and/or maintains/verifies SBOMs but to create
incentives for developers of OSS to create SMBOs (a tricky problem)} \trevor{The idea here was that SBOMs could be created by the community for projects.  Similar to how issues are tracked.  This would work for older projects that are no longer maintained}


While less than ideal, one proposed solution for improving the availability of SBOMs is opening their creation to open source. A downstream component could create an SBOM on behalf of one of its dependencies and then share that file so that other groups don't also have to create the SBOM from scratch.  This would make SBOMs available for projects that are hesitant to create them and those that are no longer maintained.  In one interview, our respondent said that "it'd be great if everybody submits them... then nobody has to keep creating them over and over and over."

While this solution is better than nothing, the problems are apparent.  A better solution would involve incorporating SBOM generation, verification and updating into build systems. 

==> contents/results/solutions/software_id_solutions.tex <==

\dmg{the solutin is not to generate them, but who will be the entity responsible for creating/maintaining those identifiers. So far these seem to be ecosystem based: github is a Universal identifier for a repo (not software). pypy for installable components (e..g binary installable), etc.
}

\trevor{We don't really offer a new solution, just bring to light existing solutions.  I would be okay saving this for the extension.  It accompanies C6} \os{ok, cut?} \MAX{I agree}
There are two possible solutions to this problem. First, Registration systems have the benefit of allowing the inclusion of additional information, but as one expert said, “I think the problem with the more registration oriented IDs is it's just not getting adopted. Or it's getting adopted in the ways that are [like] the CPEs, you know, you'll find five CPEs for the exact same software, and that can be a little confusing." 
%\nathan{Removed some filler phrases from quote. I think this is good practice, but correct me if I'm wrong (see commented out quote)}
%\trevor{That seems okay to me, I've been doing the same}

%“I think the problem with the more registration oriented IDs is there's just not, it's just not getting adopted. Or it's getting adopted in the ways that are, you know, it's like the CPEs, you know, you'll find, you know, five CPEs for the exact same software, and that can be a little confusing."

Then, there are the machine-generated IDs.  Based on the NTIA's document on SBOM versions \cite{surveyOfSBOMStandards} and our expert interviews, we have identified the five most common software identity formats.  These are:  Concise SWID Tags (CoSWID) \cite{coswid}, Common Platform Enumeration (CPE) \cite{cpe}, Package-URLs (purl) \cite{purl}, SoftWare Heritage persistent IDentifiers (SWHID) \cite{heritage}, and GitOIDs \cite{gitoid_1,gitoid_spdx}.

One interviewee discusses purl as a solution, “But it [package url] helps a lot to have a seamless way to identify a package just by observing the code, in most cases. And once you have that, it becomes easy to relate that to a security database, a dependency tree, or anything else." \MAX{drop}

As is the case with SBOM, it is unlikely that a single software identification standard will emerge or win out over the others.  Instead, we must live in a world where all the standards can successfully and harmoniously coexist. 

==> contents/results/solutions/verify_sbom_solution.tex <==
%\dmg{solution to what?}\trevor{Not being able to verify the contents of SBOMs.  I know that sounds circular or redundant, but it was a problem expressed}\nathan{Clarified the language to explicitly say what we're trying to address}
One potential means of addressing incomplete or incorrect SBOMs would be to hold parties accountable for the SBOMs they generate \ref{sec:poor_sbom}.  However, this could lead to unintended consequences.  A legal practitioner said, "[a] requirement for them to certify that it is complete or correct is only going to result in fear of creating SBOMs. `Perfect' should not be the enemy of `good.'" %Another expert echoed this sentiment: "until you [are] able to make [use] of this data practically... the consistency and the quality of this data is irrelevant." \MAX{keep one example} \nathan{cut the second quote}

%\dmg{not related to the paper but got me thinking: so why do we do SBOM if the are no tools to process SBOMs? why does the gov. expect SBOMs when there is no a single tool that will scan an SBOM and compare it against SVEs? so maybe the solution to the movitation starts here: if there are tools that make it easy to verify if my software is safe (or not) using SBOMs then I am more likely to create the info. so far it is really just like: you want a yellow piece of paper with that box of goodies I am selling? ok, here it is. Why do you want? Oh, because I am expected to ask for it. How are you going to use it? I don't know, i was just told to ask for it... }

%Further shortened and cleaned this up
%Another expert seemed on the same page, "So I think this is all too preliminary. It [is] until you [are] able to make usage of this data practically. The consistency and the quality of this data is irrelevant." \trevor{there was some broken English here, so I tried to fix it to get the point across cleanly}

Exploring the idea of legal liability further, we found that it is impractical for other reasons. SPDX SBOMs are licensed under Creative Commons 0 (CC0) \cite{spdx_data_license, creative_commons_0}, meaning no warranty is included and the producer assumes no liability.  The open-source licensing of tools protects their creators from litigation since many licenses also do not provide a warranty \cite{mit}.  According to our legal expert, issues of liability would likely only arise if proprietary software or service provided a warranty. He/she "could see there being contractually accepted liability as part of [one party agreeing to provide an accurate SBOM]." %: "...if two parties have have entered into a contract together and part of that contract... [stipulates a] contractual obligation [to] provide [the customer with] a true and accurate and complete SBOM... I could see there being contractually accepted liability as part of that." \MAX{either keep the verbatim, or the paraphrase before the verbatim, to save space} \nathan{done}

% [EXTENSION]
%\trevor{We need to hunt down the quotes for these.  They are in the interviews.  Also I think a few people mentioned them in the surveys (ML and maybe key projects)}
% Addressed: we have too many quotes already
%[EXTENSION] agreed (checkmark)
Two other solutions emerged from our surveys \ref{sec:verify_sbom}.  A third-party certification or review board could approve SBOMs and endorse them. However, "central authorities have never seemed to work too well in our industry, you know, just getting everybody to adopt it", so a more practical solution may be needed.
%The checking of SBOMs could also be open sourced.  That is that 
Alternatively, the accuracy of SBOMs could be assessed by consumers and other stakeholders, with issues found reported to the SBOM producer or posted to a central location, such as a vulnerability database.  %Ultimately, this community effort could result in better SBOMs. \MAX{remove?} \nathan{this is a bit of ediatorializing: done}



==> contents/results/usage/formats_adoption.tex <==
%When asked, all groups in our practitioner survey agreed that SBOM usage is critical in the development of software.\os{cut?}
%\nathan{done}

%SPDX and CycloneDX are the two most used SBOM formats. 
Of the 50 producers, consumers, and tool makers surveyed, 16 reported using SPDX, 8 CycloneDX, and 12 both. SWID~\cite{ntiaGlance} was used by only 5 respondents, often with other formats.  Those that consume SBOM, do so frequently. \rev{35.5\% (11/31) of participants stated they use them daily and 29\% (9/31) weekly.}  %\nathan{Find how many people were aware of both SPDX and CycloneDX, check counts for critical project survey} \trevor{Does this wording imply that they were only using one or the other or both?  Because that's not what these numbers show}. 
%\trevor{The language here is also tricky, the operative word being "using".  I updated the numbers to accurately reflect what the sentence is trying to convey. (ie only considered the practitioner survey, because no one else said they used those standards, just that they were familiar.)}
%\trevor{Let's mention the quasi sbom files here}
%Done: mentioned how most of the key project contributors who claimed to use SBOMs actually used quasi-SBOMs, highlighting the confusion around them
% \dmg{The writing, here, there and in many paragraphs, can be done more concise, while keeping all the info:
% eg. Regarding Critical survey participants, out of 22, 9 did not know about SBOMs, 7 were knew about them but did not use them. Of the remaining 6 who reported using SBOM, only one used a standard format (SPDX) while the rest used package configuration files (which Tang ...). One interviewee mentioned that in their project nobody seem to care about creating and maintaining SBOMs and that this might be due to lack of tool support for these tasks. These results seem to imply a lack of interest of maintainers of OSS projects in SBOMs.} \os{Thanks DMG!}
Of the 22 critical OSS survey participants, 9 were unfamiliar with SBOMs and 7 were aware of SBOMs, while not adopting them yet. % about them but did not use them in their projects (although they expressed familiarity with SPDX and CycloneDX). 
%Of the remaining six who reported using/producing SBOMs, only one used the SPDX format while the rest used package configuration files (\eg Maven or Node package files---\aka  "quasi-SBOMs"~\cite{tang2022towards}). 
One interviewee mentioned how the limited interest is also due to the limited tool support and the need for manually maintaining SBOMs, \rev{in line with the findings of Zahan \etal \cite{zahan2023software}.}
%that in their project nobody seem to care about creating and maintaining SBOMs and that this might be due to the lack of tool support for these tasks. These results seem to imply a lack of interest in SBOMs of maintainers of OSS projects.

%Generally, key project contributors \dmg{are these OSS developers? i think it should be "Critical" survey participants to be consistent} did not make use of SBOMs or SBOM formats. Of 22 respondents, 9 said they were unfamiliar with SBOMs and 7 claimed to be familiar with SBOMs but did not use them in their projects. Even among those who reported producing or consuming SBOMs, only one reported using a standard SBOM format, SPDX. The other respondents either reported either being unaware of SBOM formats or using package configuration files that Tang et al. describe as "quasi-SBOMs" \cite{tang2022towards}. 
%However, those who reported being aware of SBOMs but did not currently use them in their projects cited familiarity with SPDX and CycloneDX. Thus, it seems as though even when key project contributors did not mistake quasi-SBOMs for recognized SBOM formats, they were not interested in using them. One interviewee told us that they didn't think people in projects they worked on cared about having SBOMs, because no one had went to the trouble of creating or maintaining SBOMs themselves. The same person cited a lack of good tools to create and maintain SBOMs as component of this phenomenon. 

%\MAX{this paragraph needs to be moved in the results} \os{Done}
% \dmg{the comment on paywall is speculation, not mentioned by survey? so remove it, it adds
% nothing}\nathan{one interviewee explicitly mentioned that they wouldn't use swid because it was behind a paywall. But I agree that it's tough to generalize}\os{I am gonna cut this for now...}
% We found limited evidence of SWID usage, but this could be in part because the SWID specifications are hidden behind an ISO paywall \cite{swid_specification,swid_presentation}.  That said, a guide to creating SWID tags is available through the NTIA \cite{swid_guidelines}, and we found a few usages of a concise version of SWID, called coSWID \cite{coswid}, in our survey.\os{cut?} \nathan{When we first started, the fact that we couldn't find much of anything related to SWID really confused us, since it was supposedly one of the three main SBOM formats. I think this might be valuable to help prevent people from falling into that same trap. Let's see if there's space.}

% \dmg{i would rewrite the one below:
% it is possible that private organizations and closed-source projects use SBOMs--either standard formats or their own-- but this survey did not find any evidence to support this.
% (the CERN comment is not really result, it is editorializing... at best in discussion)
% }\os{Partially addressed}

It is possible that private organizations and closed-source projects use SBOMs---in any of the standard formats or their own---yet our study did not find any evidence of that. For example, it is known that CERN uses CycloneDX \cite{cern_1, cern_2} and popular standards have been mentioned by Eggers \etal for the nuclear industry \cite{eggers2022towards}.

%\trevor{Do we have more BOM usage information for cyber physical systems, maybe a brief sentence about HBOMs}
%\nathan{Added statistics and moved from use cases to adoption, since we talk more about usage here}
Of 6 CPS respondents, 3 were familiar with HBOMs and 2 had used them, but with bespoke formats.
%one used a proprietary format, and the other a c CSV file. 
\rev{No ML practitioners surveyed were aware of BOM formats for AI systems or datasets.}

==> contents/results/usage/tooling.tex <==
There was little consistency in the tools used across participants, with there being a mix of in-house, commercial (\eg Anchore \cite{anchore}), and open source solutions (\eg ScanCode \cite{scancode}).  
% \dmg{Hugginface? what is it? but this section was about tools, instead you talk about "cards" which is not a tool. or is it? but I think this needs to be answered from a higher point of view: are there tools? are they used? are they at least known? do people complain about them or are they happy with them? etc.}\os{agreed!} \MAX{sorry but I disagree! Huggingface greatly helps the distribution of ML models, especially pre-trained ones, and related datasets. It is similar to DockerHub for containers. I believe this point is extremely timely and a good addon wrt. previous studies.} \os{I actually agree to keep it.... My agreement was wiith Daniel was that we need to talk about other tooling not just ai and ml related}


\label{sec:dist}
Despite the NTIA recommendations \cite{sbom_Sharing}, there is currently no agreed-upon method for distributing SBOMs. %We asked survey respondents how they would prefer SBOMs be distributed. 
Respondents have the expectation that the developers of third-party components they use should be the ones creating, maintaining, and distributing SBOMs along with their software. % they release.  
\rev{13 (38.5\%)} critical project developers mentioned SBOM distribution as a challenge moving forward.
%This made it the largest challenge from that group.  Additionally, one respondent from the SBOM practitioner survey also mentioned distribution as a major challenge.  

%As one interviewee put it, "wherever you're getting the package, get the SBOM, too." This was consistent across all groups surveyed.

%Across all groups surveyed, the most popular response was that SBOMs should be included in repositories along with a project's source code, and the least popular option was being available upon request from the project's developers. We found that respondents generally seemed to believe that the SBOM should be located as close to the artifacts they describe as possible. As one interviewee put it, "wherever you're getting the package, get the SBOM, too." 

%\dmg{I would make it stronger: "respondents have the expectation that the developers of the dependencies should be the ones creating, maintaining and distributing SBOMs along with the software they make available. }\os{done}

%\MAX{One thing: are we only talking about tooling for AIBOM/DataBOM?} \os{We need to talk about tooling in general as well} \nathan{moved to discussion of tools in general}
Concerning support for DataBOMs and AIBOMs, two survey participants mentioned that Hugging Face dataset cards \cite{data_cards} could serve as DataBOMs.  %, while it does not directly provide tool support. 
Three respondents mentioned the same service's model cards, providing similar information to  AIBOMs.  Other tools mentioned include DVC \cite{dvc} and ML-Flow \cite{ml_flow}.  \rev{These formats fall under what we might call quasi-AIBOMs, since, to our knowledge, no formal AIBOM standards have been implemented and accepted in practice.}

%\os{Something interesting to say about when to produce SBOMs (build time, release time, etc)?}
When 34 producers were asked when SBOMs should be generated, they indicated: during each build (28), when publishing a major release~(21), during deployment (19), and at the developer's discretion (7). 

% \trevor{See this sheet for information on distribution: \url{https://docs.google.com/spreadsheets/d/1uA0NbZs4Acq5thibCLXyoBFBG92pgYfUaQPfKM6idd0/edit\#gid=1868992489}}

==> contents/results/usage/use_cases.tex <==

%"It'd be ideal if, in that one [document], you had everything you needed to know to make all your business decisions."\os{cut?}
%\nathan{done}

In line with existing SBOM documentation~\cite{ntia_benefits} and prior studies~\cite{xia2023empirical, zahan2023software}, we found that security, dependency tracking \cite{rousseau2020software}, and licensing are the main use cases for SBOMs. 
%As might be expected \cite{ntia_benefits}, survey responses indicated that security, dependency tracking, licensing are the main use cases for SBOMs. 
%When asked what the purposes of SBOMs were, 
Out of 61 SBOM practitioners, 55 mentioned as main use case dependency management, 22 licensing concerns, and 22 software security (\eg vulnerability) management.
Other responses include software versioning (14), provenance (10), documentation (6), and transparency (4).
%\MAX{the last sentence could be dropped if needed}\denys{agree}

%Respondents were also asked what they used SBOMs for. 
While tracking vulnerabilities was a main use case for \rev{consumers~(80.7\%), producers (100\%), and tool makers (83.3\%),}
some respondents were concerned that SBOMs might provide a road map of vulnerabilities for attackers.  \rev{This misconception, also identified by Zahan \etal \cite{zahan2023software}, has been addressed by NTIA \cite{myths_and_facts} and our interviewees rejected the  notion of "security by obscurity."}% as a solution.}
%\os{cut?} \MAX{I shortened, yet this point is interesting}

When 41 SBOM producers, tool makers, and standard makers were asked which fields should be included in SBOMs, responses varied. The most common answers were general information about the software components:
version number (24), license (22), component name (18), and a URL to the component (18). Notably, 13 respondents indicated that the SBOM should contain unique identifiers for the software component the SBOM is documenting and/or its dependencies~\cite{coswid, cpe, purl, heritage, gitoid_1,gitoid_spdx}.

% [EXTENSION]
%\trevor{maybe we should mention how SBOM may be a solution to the problem of license compliance when once piece of software is licensed at the file level.  Greg mentions this when talking about how they use SPDX}
% Addressed: There isn't room to include this information
% Maybe in the extension we can add a section titled problems that BOMs could solve [this use cases section could really be expanded]
% [EXTENSION]

\rev{Although we found little evidence to suggest AI and DataBOMs being used in practice, respondents mentioned two potential use cases.  These BOMs could facilitate ML model reproducibility and help to identify / verify datasets across academic papers.  Specifically, AIBOM can provide transparency into how a model was trained, providing information about its architecture, hyper-parameters, and any pre-trained base models used. By providing provenance and usage infromation, a linked DataBOM can also make developers aware if a model was trained using a poisoned, biased, or illegally sourced dataset.} %\trevor{I tried to add some more theoretical use cases for AIBOM and DataBOM to further motivate the idea}

\rev{From discussions with CPS domain experts, we identified that BOMs could serve as regulatory documents for critical embedded systems (consistent with the findings of \cite{carmody2021building}), and that they could increase the transparency and reproducibility of research results in academic circles.  For these tasks, the BOMs must communicate information related to the physical hardware components (part numbers, manufacturer, etc), firmware, and software (including configurations) of the system.}

%\dmg{is this from the respondents, or editorializing? same with next paragraph}\os{yeah, these sentences sound like our opinions} %This would be particularly impactful in the realm of academia and research.  The BOMs could serve as concise, machine-readable documentation of the model's architecture and training.
%Also, respondents indicated how AIBOMs could help to identify and verify datasets across academic papers.
%and verifying that they are actually the same.
%One practitioner commented: "sometimes you read a paper that uses a dataset A and then another paper, which claims to use dataset A, but really [the] second paper got [the dataset] from a third party [...] 
% who made a small change to it. 
% So you don't really know for sure if those two papers are using the same underlying data." \MAX{quoting is cool but can be dropped to make space}

%\MAX{no CPS/HBOM use case?}
%\denys{I was hoping for some answer demonstrating an interplay between tracking software/hardware dependencies/versions ...}

% \os{Cutting this for now...}
% \dmg{I would word these sentences backwards. It sounds like you already have an idea in your brain and are looking for support to it. Instead, you first mention the results of the survey
% and then the conclusion that you draw. Or at the very least, you say: Participants also found that ... otherwise it sounds like you have an opinion and are using the survey too support it}
% Reproducibility is also important in cyber-physical systems, and survey results indicated that understanding the configuration and limitations of a solution could greatly enhance research outcomes. \os{not sure I understand this, cut?}
% \nathan{The idea here is that people mentioned that exactly replicating test conditions is hard in complex CPS and BOMs could help w/ this, but I agree that we probably don't have the space for it here and should cut}

% [EXTENSION]
%\trevor{Talk about specific problems that require different boms ie. Saasbom}
% Addressed: This is interesting, but we don't have room for it in this paper.  We can save cloud issues for the extension
% [EXTENSION]


==> contents/tables/realtionships_challenges_solutions_roles.tex <==
\begin{table}[]
\caption{Relationships btw. challenges,  solutions, and roles.}
\label{tab:challenges}
\setlength{\tabcolsep}{2pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c}
\hline
\textbf{Challenge}               & \textbf{Solved by }                      & \textbf{Depends on}                                                                           & \textbf{Affected}               & \textbf{Who can fix it} \\ \hline
\multicolumn{1}{c|}{C1}  & \multicolumn{1}{c|}{S1}         & \multicolumn{1}{c|}{C2, C3}                                                          & \multicolumn{1}{c|}{P, C, TM} & SM, E          \\
\multicolumn{1}{c|}{C2}  & \multicolumn{1}{c|}{S1}         & \multicolumn{1}{c|}{C9}                                                              & \multicolumn{1}{c|}{P, C, TM} & SM             \\
\multicolumn{1}{c|}{C3}  & \multicolumn{1}{c|}{S2}         & \multicolumn{1}{c|}{-}                                                               & \multicolumn{1}{c|}{P, C, TM} & SM             \\
\multicolumn{1}{c|}{C4}  & \multicolumn{1}{c|}{S2}         & \multicolumn{1}{c|}{C5}                                                              & \multicolumn{1}{c|}{P, C}     & P, TM          \\
\multicolumn{1}{c|}{C5}  & \multicolumn{1}{c|}{S2, S4}     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}C1,C2,C3,\\ C6,C7\end{tabular}}       & \multicolumn{1}{c|}{P, C}     & TM             \\
\multicolumn{1}{c|}{C6}  & \multicolumn{1}{c|}{S1, S2, S3} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}C4, C5, C9,\\  C10, C11\end{tabular}} & \multicolumn{1}{c|}{P, C, TM} & P, TM          \\
\multicolumn{1}{c|}{C7}  & \multicolumn{1}{c|}{S2, S3}     & \multicolumn{1}{c|}{C6}                                                              & \multicolumn{1}{c|}{C}        & TM             \\
\multicolumn{1}{c|}{C8}  & \multicolumn{1}{c|}{S1, S2}     & \multicolumn{1}{c|}{C5}                                                              & \multicolumn{1}{c|}{P}        & TM             \\
\multicolumn{1}{c|}{C9}  & \multicolumn{1}{c|}{S1}         & \multicolumn{1}{c|}{-}                                                               & \multicolumn{1}{c|}{P, C}     & SM, TM         \\
\multicolumn{1}{c|}{C10} & \multicolumn{1}{c|}{-}          & \multicolumn{1}{c|}{-}                                                               & \multicolumn{1}{c|}{P}        & -              \\
\multicolumn{1}{c|}{C11} & \multicolumn{1}{c|}{-}          & \multicolumn{1}{c|}{C8}                                                              & \multicolumn{1}{c|}{P}        & -              \\
\multicolumn{1}{c|}{C12} & \multicolumn{1}{c|}{S4}         & \multicolumn{1}{c|}{C1, C3}                                                          & \multicolumn{1}{c|}{P, C}     & SM, E  \\       \hline
\end{tabular}
}
{\footnotesize Role: P=Producer, C=Consumer, TM=Tool Maker, E=Educator, SM=Standard Maker}
\vspace{-0.3cm}
\end{table}

==> contents/tables/solutions_to_challenges.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\caption{Challenge / solution mapping}
\label{tab:solutions}
\begin{tabular}{| p{0.18\linewidth} | p{0.28\linewidth}| p{0.35\linewidth} | p{0.075\linewidth}|}
\hline
Solution & Challenges Addressed & How? & Impacted \\ \hline
\multirow{4}{1\linewidth}{(S1) Multi-dimensional SBOM specifications} & (C1) Complexity of SBOM specifications & Specifications for a particular type of software or use case will be shorter and not clutter with seemingly superfluous information & P, C, TM \\ \cline{2-4} 
 & (C2) Determining data fields to include in SBOMs & New fields can be added for special use cases without cluttering the spec for other cases & P, C, TM \\ \cline{2-4} 
 & (C6) Inaccurate and incomplete SBOMs & SBOMs will be less likely to be incomplete if information that is hard to find or irrelevant isn't required & P, C, TM \\ \cline{2-4} 
 & (C9) SBOM completeness and data privacy trade-off & Specifications can tailor the required fields for this specific scenario & P, C \\ \hline
\multirow{5}{1\linewidth}{(S2) Enhanced SBOM tooling and build system support} & (C4) Keeping SBOMs up to date & Proper tooling should be compatible with continuous integration and able to automatically update SBOMs, keeping them up to date with the project & P, C \\ \cline{2-4} 
 & (C5) Insufficient SBOM tooling & Improved tool support will trivially address the problem of insuffiecent tooling & P, C \\ \cline{2-4} 
 & (C6) Inaccurate and incomplete SBOMs & Tools that are sufficient should generate accurate and complete SBOMs, perhaps through improved scanners or manifest checking & P, C, TM \\ \cline{2-4} 
 & (C7) Verifying SBOM accuracy and completeness & Good SBOM consumption tools will be able to evaluate the quality of an SBOM & C \\ \cline{2-4} 
 & (C8) Differences across ecosystems and communities & More tools and additional build system support will enable SBOM use across languages and ecosystems & P \\ \hline
\multirow{2}{1\linewidth}{(S3) Strategies for SBOM verification} & (C6) Inaccurate and incomplete SBOMs & With verification systems in place, certified SBOMs will be accurate and complete & P, C, TM \\ \cline{2-4} 
 & (C7) Verifying SBOM accuracy and completeness & By verifying the contents of an SBOM, it's accuracy and completeness has been checked & C \\ \hline
\multirow{2}{1\linewidth}{(S4) Increasing incentives for SBOM adoption} & (C5) Insufficient SBOM tooling & Increased incentive will drive further open source tool creation & P, C \\ \cline{2-4} 
 & (C12) Unclear SBOM direction & Further involvement from the open source community will help clarify and strengthen the direction of SBOM usage & P, C \\ \hline
\end{tabular}%
\end{table}
